The Lx-Yx Relation: Using Galaxy Cluster X-Ray Luminosity as a Robust, Low Scatter Mass Proxy

We use a sample of 115 galaxy clusters at 0.1<z<1.3 observed with Chandra ACIS-I to investigate the relation between luminosity and Yx (the product of gas mass and temperature). The scatter in the relation is dominated by cluster cores, and a tight LY relation (11% intrinsic scatter in Lx) is recovered if sufficiently large core regions (0.15R500) are excluded. The intrinsic scatter is well described by a lognormal distribution and the relations are consistent for relaxed and disturbed/merging clusters. We investigate the LY relation in low-quality data (e.g. for clusters detected in X-ray survey data) by estimating Lx from soft band count rates, and find that the scatter increases somewhat to 21%. We confirm the tight correlation between Yx and mass and the self-similar evolution of that scaling relation out to z=0.6 for a subset of clusters in our sample with mass estimates from the literature. This is used to estimate masses for the entire sample and hence measure the LM relation. We find that the scatter in the LM relation is much lower than previous estimates, due to the full removal of cluster cores and more robust mass estimates. For high-redshift clusters the scatter in the LM relation remains low if cluster cores are not excluded. These results suggest that cluster masses can be reliably estimated from simple luminosity measurements in low quality data where direct mass estimates, or measurements of Yx are not possible. This has important applications in the estimation of cosmological parameters from X-ray cluster surveys.

==> newcom.tex <==
% LaTeX2e new commands file (adapted from LaTeX definitions file)
%  Modified by Alastair Sanderson
% Created: 16-7-01 by Dave Henley
% Last modified: 20-7-01  AJRS
% modified by BJM 9/8/01 - added more units

% Common physical/astrophysical symbols
\newcommand{\Fx}{\ensuremath{F_{\mathrm{X}}}}
\newcommand{\Fxobs}{\ensuremath{F_{\mathrm{X}}^{\mathrm{obs}}}}
\newcommand{\Halpha}{H$\alpha$}
\newcommand{\Lbol}{\ensuremath{L_{\mathrm{bol}}}}
\newcommand{\Lsol}{\ensuremath{L_{\odot}}}
\newcommand{\Lx}{\ensuremath{L_{\mathrm{X}}}}
\newcommand{\Yx}{\ensuremath{Y_{\mathrm{X}}}}
\newcommand{\Ysz}{\ensuremath{Y_{\mathrm{SZ}}}}
\newcommand{\Napec}{\ensuremath{N_{\mathrm{APEC}}}}
\newcommand{\Lyalpha}{Ly$\alpha$}
\newcommand{\Lybeta}{Ly$\beta$}
\newcommand{\Lygamma}{Ly$\gamma$}
\newcommand{\mH}{\ensuremath{m_{\mathrm{H}}}}
\newcommand{\Mdot}{\ensuremath{\dot{M}}}
\newcommand{\Msol}{\ensuremath{\mathrm{M_{\odot}}}}
\newcommand{\Ne}{\ensuremath{n_{\mathrm{e}}}}
\newcommand{\NH}{\ensuremath{N_{\mathrm{H}}}}
\newcommand{\NHe}{\ensuremath{N_{\mathrm{He}}}}
\newcommand{\Rsol}{\ensuremath{\mathrm{R_{\odot}}}}
\newcommand{\Rstar}{\ensuremath{R_{\ast}}}
\newcommand{\RV}{\ensuremath{R_{\mathrm{v}}}}
\newcommand{\Dv}{\ensuremath{\Delta_{\mathrm{v}}}}
\newcommand{\rt}{\ensuremath{R_{\mathrm{200}}}}
\newcommand{\rf}{\ensuremath{R_{\mathrm{500}}}}
\newcommand{\rn}[1]{\ensuremath{R_{\mathrm{#1}}}}
\newcommand{\rc}{\ensuremath{r_{\mathrm{c}}}}
\newcommand{\rd}{\ensuremath{r_{\mathrm{d}}}}
\newcommand{\rxsig}[1]{\ensuremath{r_{#1\sigma}}}
%\def\R200{\ensuremath{R_{\mathrm{200}}}}
%\def\r200{\ensuremath{r_{\mathrm{200}}}}
%won't work%\newcommand{\R200}{\ensuremath{R_{\mathrm{200}}}}
\newcommand{\Mf}{\ensuremath{M_{\mathrm{500}}}}
\newcommand{\Mt}{\ensuremath{M_{\mathrm{200}}}}
\newcommand{\Tx}{\ensuremath{T_{\mathrm{X}}}}
\newcommand{\Zsol}{\ensuremath{\mathrm{Z_{\odot}}}}
\newcommand{\fgas}{\ensuremath{f_{\mathrm{gas}}}}
\newcommand{\Mgas}{\ensuremath{M_{\mathrm{gas}}}}
\newcommand{\Om}{\ensuremath{\Omega_{\mathrm{m}}}}
\newcommand{\OM}{\ensuremath{\Omega_{\mathrm{M}}}}
\newcommand{\Or}{\ensuremath{\Omega_{\mathrm{r}}}}
\newcommand{\OR}{\ensuremath{\Omega_{\mathrm{R}}}}
\newcommand{\Ob}{\ensuremath{\Omega_{\mathrm{b}}}}
\newcommand{\OB}{\ensuremath{\Omega_{\mathrm{B}}}}
\newcommand{\zo}{\ensuremath{z_{\mathrm{obs}}}}
\newcommand{\zf}{\ensuremath{z_{\mathrm{form}}}}


% Text abbreviations
\newcommand{\eg}{{\it e.g.\ }}
\newcommand{\egc}{{\it e.g.}}  % Citation version; no space afterwards
\newcommand{\etal}{et al.\ }
\newcommand{\etc}{{\it etc.\ }}
\newcommand{\cf}{{\it c.f.\ }}
\newcommand{\ie}{{\it i.e.\ }}


% Proper nouns
\newcommand{\ASCA}{\emph{ASCA}}
\newcommand{\Chandra}{\emph{Chandra}}
\newcommand{\Einstein}{\emph{Einstein}}
\newcommand{\ROSAT}{\emph{ROSAT}}
\newcommand{\XMM}{\emph{XMM-Newton}}
\newcommand{\Ariel}{\emph{Ariel 5}}
\newcommand{\Uhuru}{\emph{Uhuru}}
\newcommand{\BeppoSAX}{\emph{BeppoSAX}}
\newcommand{\MEKAL}{\textsc{MeKaL}}


% Maths symbols
\newcommand{\chisq}{\ensuremath{\chi^2}}
\newcommand{\rchisq}{\ensuremath{\chi^2_\nu}}
\newcommand{\gta}{\,\rlap{\raise 0.4ex\hbox{$>$}}{\lower 0.6ex\hbox{$\sim$}}\,}  
\newcommand{\lta}{\,\rlap{\raise 0.4ex\hbox{$<$}}{\lower 0.6ex\hbox{$\sim$}}\,}  

% Simple units
% Length
\newcommand{\angstrom}{\mbox{\ensuremath{\mathrm{~\AA}}}}
\newcommand{\nm}{\mbox{\ensuremath{\mathrm{~\nm}}}}
\newcommand{\mymicron}{\mbox{\ensuremath{\mathrm{~\mu m}}}}
\newcommand{\cm}{\mbox{\ensuremath{\mathrm{~cm}}}}
\newcommand{\m}{\mbox{\ensuremath{\mathrm{~m}}}}
\newcommand{\km}{\mbox{\ensuremath{\mathrm{~km}}}}
\newcommand{\AU}{\mbox{\ensuremath{\mathrm{~A.U.}}}}
\newcommand{\pc}{\mbox{\ensuremath{\mathrm{~pc}}}}
\newcommand{\kpc}{\mbox{\ensuremath{\mathrm{~kpc}}}}
\newcommand{\Mpc}{\mbox{\ensuremath{\mathrm{~Mpc}}}}
% Time
\newcommand{\s}{\mbox{\ensuremath{\mathrm{~s}}}}
\newcommand{\ks}{\mbox{\ensuremath{\mathrm{~ks}}}}
\newcommand{\hour}{\mbox{\ensuremath{\mathrm{~hour}}}}
\newcommand{\yr}{\mbox{\ensuremath{\mathrm{~yr}}}}
\newcommand{\Gyr}{\mbox{\ensuremath{\mathrm{~Gyr}}}}
% Mass
\newcommand{\gram}{\mbox{\ensuremath{\mathrm{~g}}}}
% Energy
\newcommand{\eV}{\mbox{\ensuremath{\mathrm{~eV}}}}
\newcommand{\keV}{\mbox{\ensuremath{\mathrm{~keV}}}}
\newcommand{\erg}{\mbox{\ensuremath{\mathrm{~erg}}}}
\newcommand{\Hz}{\mbox{\ensuremath{\mathrm{~Hz}}}}
\newcommand{\kHz}{\mbox{\ensuremath{\mathrm{~kHz}}}}
\newcommand{\GHz}{\mbox{\ensuremath{\mathrm{~GHz}}}}
% Angle
\newcommand{\degree}{\ensuremath{\mathrm{^\circ}}}
\newcommand{\arcm}{\ensuremath{\mathrm{^\prime}}}
\newcommand{\arcs}{\arcm\hskip -0.1em\arcm}
\newcommand{\dotarcs}{\,\rlap{\hbox{$\mathrm{^\prime\hskip -0.1em^\prime}$}}{\hbox{$.$}}\,}
\newcommand{\dotsec}{\,\rlap{\hbox{$\mathrm{^s}$}}{\hbox{$.$}}\,}
% Misc.
\newcommand{\gauss}{\mbox{\ensuremath{\mathrm{~G}}}}
\newcommand{\kelvin}{\mbox{\ensuremath{\mathrm{~K}}}}
\newcommand{\K}{\mbox{\ensuremath{\mathrm{~K}}}}
\newcommand{\photons}{\mbox{\ensuremath{\mathrm{~photons}}}}
\newcommand{\mags}{\mbox{\ensuremath{\mathrm{~mag}}}}
\newcommand{\C}{\mbox{\ensuremath{~\degree\mathrm{C}}}}


% Compound units
\newcommand{\cmsq}{\ensuremath{\mathrm{\cm^2}}}
\newcommand{\cc}{\ensuremath{\mathrm{\cm^3}}}
\newcommand{\pcc}{\ensuremath{\mathrm{\cm^{-3}}}}
\newcommand{\gpcc}{\ensuremath{\mathrm{\gram\cm^{-3}}}}
\newcommand{\pcmsq}{\mbox{\ensuremath{\mathrm{~cm^{-2}}}}}
\newcommand{\pMpc}{\ensuremath{\mathrm{\Mpc^{-1}}}}
\newcommand{\ps}{\ensuremath{\mathrm{\s^{-1}}}}
\newcommand{\pyr}{\ensuremath{\mathrm{\yr^{-1}}}}

\newcommand{\cmps}{\ensuremath{\mathrm{\cm \ps}}}
\newcommand{\ctps}{\ensuremath{\mathrm{ ~counts \ps}}}
\newcommand{\ctpp}{\ensuremath{\mathrm{ ~counts ~pixel^{-1}}}}
\newcommand{\arcpp}{\ensuremath{\mathrm{\arcs ~pixel^{-1}}}}
\newcommand{\ctpsqaps}{\ensuremath{\mathrm{ ~counts ~arcsec^{-2} \ps}}}
\newcommand{\ergps}{\ensuremath{\mathrm{\erg \ps}}}
\newcommand{\flux}{\ensuremath{\mathrm{\erg \ps \pcmsq}}}
\newcommand{\ent}{\ensuremath{\mathrm{\keV \cmsq}}}
\newcommand{\kmps}{\ensuremath{\mathrm{\km \ps}}}
\newcommand{\kmpspMpc}{\ensuremath{\mathrm{\km \ps \pMpc\,}}}
\newcommand{\LT}{\mbox{\ensuremath{\mathrm{L_{X}-kT}}}}
\newcommand{\YL}{\mbox{\ensuremath{\mathrm{Y_{X}-L_{X}}}}}
\newcommand{\LY}{\mbox{\ensuremath{\mathrm{L_{X}-Y_{X}}}}}
\newcommand{\YM}{\mbox{\ensuremath{\mathrm{Y_{X}-M_{500}}}}}
\newcommand{\LM}{\mbox{\ensuremath{\mathrm{L_X-M}}}}
\newcommand{\LMf}{\mbox{\ensuremath{\mathrm{L_X-M_{500}}}}}
\newcommand{\ML}{\mbox{\ensuremath{\mathrm{M-L_X}}}}
\newcommand{\MgL}{\mbox{\ensuremath{\mathrm{M_{gas}-L_{X}}}}}
\newcommand{\Msolpy}{\mbox{\ensuremath{\mathrm{ } \Msol \pyr}}}
\newcommand{\MnT}[1]{\mbox{\ensuremath{\mathrm{M_{#1}-T}}}}
\newcommand{\LnT}[1]{\mbox{\ensuremath{\mathrm{L_{#1}-T}}}}
\newcommand{\MT}{\mbox{\ensuremath{\mathrm{M-kT}}}}
\newcommand{\MgT}{\mbox{\ensuremath{\mathrm{M_{g}-kT}}}}



% Ionization states
%\newcommand{\CaXIX}{Ca~\textsc{xix}}
%\newcommand{\FeXVII}{Fe~\textsc{xvii}}
%\newcommand{\FeXVIII}{Fe~\textsc{xviii}}
%\newcommand{\FeXX}{Fe~\textsc{xx}}
%\newcommand{\FeXXV}{Fe~\textsc{xxv}}
%\newcommand{\MgX}{Mg~\textsc{x}}
%\newcommand{\MgXI}{Mg~\textsc{xi}}
%\newcommand{\MgXII}{Mg~\textsc{xii}}
%\newcommand{\NVI}{N~\textsc{vi}}
%\newcommand{\NVII}{N~\textsc{vii}}
%\newcommand{\NeIX}{Ne~\textsc{ix}}
%\newcommand{\NeX}{Ne~\textsc{x}}
%\newcommand{\OIV}{O~\textsc{iv}}
%\newcommand{\OVI}{O~\textsc{vi}}
%\newcommand{\OVII}{O~\textsc{vii}}
%\newcommand{\OVIII}{O~\textsc{viii}}
%\newcommand{\SXV}{S~\textsc{xv}}
%\newcommand{\SXVI}{S~\textsc{xvi}}
%\newcommand{\SiXIII}{Si~\textsc{xiii}}
%\newcommand{\SiXIV}{Si~\textsc{xiv}}

% Miscellaneous
\newcommand{\To}{--}
\newcommand{\LCDM}{$\Lambda$CDM~}

